Bullwhip Effect of Supply Networks: Joint Impact of Network Structure and Market Demand

The progressive amplification of fluctuations in demand as the demand travels upstream the supply chains is known as the bullwhip effect. We first analytically characterize the bullwhip effect in general supply chain networks in two cases: (i) all suppliers have a unique layer position, where our method is founded on the control-theoretic approach, and (ii) not all suppliers have a unique layer position due to the presence of intra-layer links or inter-layer links between suppliers that are not positioned in consecutive layers, where we use both the absorbing Markov chain and the control-theoretic approach. We then investigate how network structures impact the BWE of supply chain networks. In particular, we analytically show that (i) if the market demand is generated from the same stationary process, the structure of supply networks does not affect the layer-wise bullwhip effect of supply networks, and (ii) if the market demand is generated from different stationary or non-stationary market processes, wider supply networks lead to a lower level of layer-wise bullwhip effect. Finally, numerical simulations are used to validate our propositions.

==> c-notes.tex <==
Demand modeling:

``We assume an underlying AR(1) demand process (AR(1)) con
sistent
with Kahn (1987), Lee et al. (1997), Chen et al. (2000a,b),
and Luong (2007). Doing so creates a basis for considering other
demand processes in future work, building on the step demand
by Warburton (2004); AR(p) demand by Chandra and Grabis
(2005) and Luong and Phien (2007); ARMA demand by Duc et al.
(2008); ARIMA by Gilbert (2005); and general demand by Ouyang
and Daganzo (2008).``

Measuring the bullwhip effect for supply chains with seasonal demand components：  the relationship between lead-time and seasonal lags are crucial to bullwhip effect reduction

Evolution of ARMA demand in supply chains. MOSM 2004

Gilbert, K., 2005. An arima supply chain model. Management Science 51, 305–310

``Most research in this direction has assumed that demand is a stochastic process. The simplest demand model is an independently and identically distributed (i.i.d.) Gaussian white noise process (Deziel & Eilon, 1967). This model has some mathematical advantages, but may be an over-simplification as it overlooks temporal correlation in the demand signal. Demand correlation can be accounted for with auto-regressive integrated moving average (ARIMA) models (Box & Jenkins, 1970). The first order auto-regressive demand model, AR(1), has perhaps been the most frequently adopted (Chen, Dresner, Ryan and Simchi-Levi, 2000a, Lee, Padmanabhan and Whang, 1997, Lee, So and Tang, 2000, amongst others). This demand model has only one parameter, so it is easy to observe the impact of autocorrelation without sacrificing too much tractability. It has been shown that positive (negative) correlation in demand increases (mitigates) bullwhip (Duc, Luong, & Kim, 2008a) and that there is an auto-regressive parameter with maximal bullwhip for a given lead time (Babai, Boylan, Syntetos, & Ali, 2015). For positive correlation, bullwhip increases with the lead time until it reaches an upper bound (Luong, 2007).

More complex ARIMA models for demand have also been studied: AR(2), AR(p) (Luong & Pien, 2007); ARMA(1,1) (Alwan, Liu, & Yao, 2003); ARMA(2,2) (Gaalman & Disney, 2009); and ARMA(p,q) (Gaalman, 2006). For non-stationary ARIMA models, since the variance of non-stationary time series is no longer finite, alternative bullwhip measures and approaches have to be adopted e.g. the variance of production changes (Graves, 1999, Miyaoka and Hausman, 2004). Demand can also be modeled using the Martingale Method of Forecast Evolution (MMFE), which generalises i.i.d., ARMA and Brownian processes. The bullwhip effect problem under MMFE demand was considered in Chen and Lee (2009).``

constant replenish lead time \citep{sodhi2011incremental}
